MolNexTR: A Generalized Deep Learning Model for Molecular Image Recognition

In the field of chemical structure recognition, the task of converting molecular images into machine-readable data formats such as SMILES string stands as a significant challenge, primarily due to the varied drawing styles and conventions prevalent in chemical literature. To bridge this gap, we proposed MolNexTR, a novel image-to-graph deep learning model that collaborates to fuse the strengths of ConvNext, a powerful Convolutional Neural Network variant, and Vision-TRansformer. This integration facilitates a more detailed extraction of both local and global features from molecular images. MolNexTR can predict atoms and bonds simultaneously and understand their layout rules. It also excels at flexibly integrating symbolic chemistry principles to discern chirality and decipher abbreviated structures. We further incorporate a series of advanced algorithms, including an improved data augmentation module, an image contamination module, and a post-processing module for getting the final SMILES output. These modules cooperate to enhance the model's robustness to diverse styles of molecular images found in real literature. In our test sets, MolNexTR has demonstrated superior performance, achieving an accuracy rate of 81-97%, marking a significant advancement in the domain of molecular structure recognition.

==> sections/1_abstract.tex <==
% ----------------------------------------
\section{abstract}
In the dynamic field of molecular structure recognition, the task of converting molecular images into graph structures and SMILES strings stands as a significant challenge, primarily due to the varied drawing styles and conventions prevalent in chemical literature. 
To bridge this gap, we proposed MolNextTR, a novel image-to-graph model that collaborates to fuse the strengths of a Convolutional Neural Network, ConvNext, and TRansformer. 
This integration facilitates a more nuanced extraction of both local and global features from molecular images.
MolNexTR excels at flexibly integrating symbolic chemistry principles to discern chirality and decipher abbreviated structures.
We further incorporate a series of advanced algorithms, including improved data augmentation module, image contamination module, and post-processing modules. 
These algorithms synergistically enhance the model's robustness against the diverse styles of molecular imagery found in real literature. 
In public benchmark tests, MolNexTR has demonstrated superior performance, achieving an accuracy rate of 81-97\%, marking a significant advancement in the domain of molecular structure recognition.

